Adversarial Testing for Visual Grounding via Image-Aware Property Reduction

Due to the advantages of fusing information from various modalities, multimodal learning is gaining increasing attention. Being a fundamental task of multimodal learning, Visual Grounding (VG), aims to locate objects in images through natural language expressions. Ensuring the quality of VG models presents significant challenges due to the complex nature of the task. In the black box scenario, existing adversarial testing techniques often fail to fully exploit the potential of both modalities of information. They typically apply perturbations based solely on either the image or text information, disregarding the crucial correlation between the two modalities, which would lead to failures in test oracles or an inability to effectively challenge VG models. To this end, we propose PEELING, a text perturbation approach via image-aware property reduction for adversarial testing of the VG model. The core idea is to reduce the property-related information in the original expression meanwhile ensuring the reduced expression can still uniquely describe the original object in the image. To achieve this, PEELING first conducts the object and properties extraction and recombination to generate candidate property reduction expressions. It then selects the satisfied expressions that accurately describe the original object while ensuring no other objects in the image fulfill the expression, through querying the image with a visual understanding technique. We evaluate PEELING on the state-of-the-art VG model, i.e. OFA-VG, involving three commonly used datasets. Results show that the adversarial tests generated by PEELING achieves 21.4% in MultiModal Impact score (MMI), and outperforms state-of-the-art baselines for images and texts by 8.2%--15.1%.

==> sec/backup.tex <==
\begin{abstract}

Due to the advantages of fusing information from various modalities, multimodal learning is gaining increasing attention. 
Being a fundamental task of multimodal learning, Visual Grounding (VG), aims to locate objects in images through natural language expressions. 
Existing metamorphic testing techniques do not make the utmost of the two modes of information, i.e. apply the perturbation based solely on the information from either the image or text, and the generated tests either cause the test oracle unknown or could not effectively challenge the model, which limits its issue detection capability.
% a single aspect of images or text for perturbation.
% Apply the perturbation based solely on the input from either the image or text end
% Due to ignoring the semantic relevance of the two aspects in the VG task, the tests generated by the previous approaches either cause the test oracle changed or could not effectively challenge the model, which limits their usability and issue detection ability.

% has been garnering increased attention due to its advantages in effectively fusing information from multiple data sources and enhancing representation learning across various modalities.
% As a fundamental task within the multimodal learning field, Visual Grounding (VG) aims to locate objects in images through natural language expressions. 
% This task has gained considerable interest in recent years, and concerns about its quality have emerged during practical applications.
% due to the development of multimodal learning.
% The quality concerns of VG models have also garnered increasing attention. 



% However, no automatic testing approach currently exists for VG models.
% Traditional testing methods for multimodal models have limited capabilities in detecting issues with VG models, as they only consider single-mode information.
% To tackle this challenge, 
% \yang{To this end, we propose {\tool}, an image-aware text perturbation approach for VG testing that could transform the expressions from comprehensive to concise under the premise that the target objects can be correctly located.}
To this end, we propose {\tool}, an image-aware text perturbation approach for VG testing, which conducts the perturbation considering both the text and the image. 
The core idea is to transform the original comprehensive expression into a concise one meanwhile keeping the described object on the image unchanged.
% (with visual understanding). 
% The concise expression involves less information and would demonstrate higher uncertainty according to Shannon's Entropy theory, therefore 
{\tool} conducts the object/property extraction and recombination to generate candidate concise expressions.
\yuan{
It then chooses the satisfied expressions that accurately describe the original object, ensuring that no other objects fit the description, by querying the image with a visual understanding technique.
}
\yang{comment.}
% 1. 
% It then selects satisfactory expressions that accurately describe the original object, ensuring that no other objects fit the description, by employing an image querying process through a visual understanding technique
% Under the framework of the metamorphic testing, {\tool} designs two metamorphic relations for the expressions.
% On the one hand, {\tool} could transform the expressions from comprehensive to concise under the premise that the concise expression still uniquely refers to the target object in the image, with the help of object/property extraction and recombination, as well as image-aware expression selection.
% On the other hand, {\tool} conducts the semantically-equivalent perturbations to further improve its issue detection ability.
We evaluate {\tool} on the state-of-the-art VG model (OFA) involving three public datasets.
Results show that, with the tests generated by {\tool}, the relative performance drop of OFA achieves 21.4\% in MultiModal Impact score (MMI), and outperforms state-of-the-art baselines for images and texts by 8.2\%-15.1\%.
\yang{comment.}
%这个relative performance drop怎么理解，是common的表达么，尤其是relative应该是表达扰动前后的性能相对值吧？感觉有点难理解。如果MMI是通用指标，直接说MMI是否可以？不提relative performance drop。
% \jie{comment}
Additionally, by fine-tuning the original model with the generated tests, the performance of OFA could be improved by 18.2\%-35.8\% in accuracy.
%这里有点乱，accuracy，和 issue detection rate是两个指标吗？两个都比基线好吗？
%要不要两个都各自说下，具体是多少，比基线好了多少。
%这部分就是太长了，简化下。
% we propose {\tool}, an image-aware text perturbation approach for automated testing VG models.
% {\tool} is the first approach to combine image and text information for metamorphic testing. 
% The core idea is that the VG model should locate the original target region on the image if we could find a concise expression that describes the original object and there are no other objects on the image that satisfy the description.
% Specifically, {\tool} (1) extracts objects and corresponding properties from the original expression; (2) reorganizes objects and properties into candidate concise representations; (3) selects appropriate concise expressions by understanding the semantics of the image with the aid of VQA model; (4) puts concise expression through semantically-equivalent perturbations to generate test suite.
% \yang{
% To evaluate the performance of {\tool}, we introduce a state-of-the-art VG model, OFA, as the tested object, and the expressions in three public datasets for the VG task as the input of metamorphic relations in {\tool}.
% }
% \yang{
% Evaluation results show that {\tool} shows the advantages in both the correct rate of generated tests and issue detection ability.
% % Specifically, the tests generated by {\tool} could reach 65.9\% in accuracy. 
% Especially, with the tests generated by {\tool}, the performance of OFA reduces 21.3\% in accuracy and outperforms state-of-the-art baselines for images and texts by 9.4\%-19.3\% in issue detection rate.
% }
% % Evaluation on three public datasets shows that {\tool} could reduce the accuracy of the VG model by 11.7\%-26.5\%, and significantly outperforms state-of-the-art baselines by 11.1\%-19.3\% in accuracy. 
% \yang{
% Additionally, by fine-tuning the original model with the generated test, the performance of OFA could be improved by 14.6\% in accuracy.
% }
% \jie{comment}
%我觉得最前面可能还是先说一句半句的multimodal learning更好一些，就说multimodel learning由于其XX方面的优势受到了越来越多的关注，或得到了广泛应用。然后说VG作为其中的重要代表什么的，具体是做什么的。要不你后面说的oriented to a single aspect 就感觉和前面的对应得不太好。有multimodel那句，就感觉会对应的比较好一些。
%第二个小问题是，as well as VQA-based test selection，在前面都没有出现test，这里叫做test selection显得有些突兀了吧？
%unpredictable or relatively shallow，感觉都一眼看不出意思来，改成这样？previous approaches  either cause the test oracle changed or couldnot effectively challenge the model ? 
%premise that the target objects can be still correctly located in the images 这个说法不太对，这个object肯定一直是locate 在images上面的，这个事情不管怎么变文本，他都不变，应该是说，这个描述还是唯一的对应这个target object，或者之类的。
%with the help of entity extraction, object and property recombination，这里entity extraction感觉和后面对应不起来，改为 with the help of object/property extraction and recombination ？
%后面的VQA要给出全称吗
% In addition, the performance of the VG model could be significantly improved by fine-tuning the original model with the generated test suite.
\end{abstract}


% \begin{IEEEkeywords}

% \end{IEEEkeywords}
\keywords{Visual Grounding, Text Perturbation, Metamorphic Testing}


\section{Introduction}
\label{sec:introduction}

%%%%% 
%1. VG很重要
%2.VG的质量问题，引出需要自动方法去测试，以往方法通过变异、突变的方式去做
%3.图片作为VG任务重要的输入，但存在XXX的问题；
%4.文字作为另一个重要输入，它和image相比，具有更多的不确定性和模糊性，对文本的变异，对于检测VG模型的质量问题的检测是一个途径；
%5.已有的方法都是等价信息的变异，需要补充；
%6.距离说明，再次任务下，可以通过信息量的删减，来进行测试；
%7.删减的时候，需要image-aware
%8.引出方法。
%%%


%%%
% logic line of Introduction. revised version 2023.3.14
% 1. VG是一个什么样的任务（重点强调VG任务的输入），VG很重要；
% 2. VG的质量问题，引出需要自动化方法去检测缺陷；
% 3. 作为VG一个重要的输入，expression的表述对VG models的性能有显著影响；
% 4. 引出一下有concise和precise的表达，说一下在VG任务下，consise和precise的定义是什么（比如有大于一个有判别性的features的expression叫做precise，只有唯一的判别性特征的expression是concise的）。举个例子说明VG model在处理concise和precise的expressions时候，性能有比较明显的差异（当然，如果有统计数据的支撑，更有说服力。如果没有的话，就用举例子的方式说吧）；
% 5. 进而引出，对于precise expressions，采用自动化的手段将其变为concise expression，是一个对于isssue detection是一个很好的路径；
% 6.引出方法，常规套路写。
%%%

%1. 多模态任务的描述
\begin{figure}[htbp]
\centering
\includegraphics[width=0.55\textwidth]{fig/motivation.png}
\caption{Comprehensive and concise expressions for VG
%这个图感觉可以稍微再美化下，感觉是不是image就只要这个大图就行了。然后下面锁边让comprehensive (original) experession 我感觉可以用个括号或者什么的，标注下是原始的，然后右边就是concise expression。
}
\label{fig:motivation}
\end{figure}

Multimodal learning is a machine-learning paradigm that leverages a variety of different data modes to train the models, including text, images, audio, and so on~\cite{zubatiuk2021development,tsai2019multimodal,gao2020survey}.
With wide applications in daily life, 
multimodal learning has attracted increasing attention in recent years~\cite{zubatiuk2021development,tsai2019multimodal,gao2020survey}.
Unfortunately, like other deep learning models, quality issues have also emerged during the application of multimodal models, which significantly reduces their reliability.
% , such as robustness and security, \jie{comment}
%感觉是不是不要提robustness and security，前者在深度学习测试领域有确定的定义，偏公式推导那种，这里写着怕引起reviewer不必要的关注。后者我们也没有关注不了。
In addition, compared to traditional single-mode deep learning models, quality issues of multimodel models can usually cause more severe impact, and greater challenges in detecting them due to the heterogeneity of model input \cite{BaltrusaitisAM19,abs-2209-03430,liang2022foundations}.
However, the automatic testing techniques for multimodal models have not been well studied, and are badly desired in real-world practice.

% \jie{fell like not `in literature', in real-world practice?}. 




% Multimodal learning has attracted increasing attention in recent years, and more and more multimodal models are widely used in people's daily life\cite{zubatiuk2021development,tsai2019multimodal,gao2020survey}.
% However, due to the heterogeneity of the multimodal model input data (i.e., image and text), models are often vulnerable under distribution shifts\cite{BaltrusaitisAM19,abs-2209-03430,liang2022foundations}.
% Therefore, a large amount of test methods have been proposed to test the robustness of the mutimodal model.
% Specifically, researchers design test methods under single-modal information, respectively.
% For image information, existing computer vision testing methods usually perturb image properties, such as pixels, luminance, etc.  \cite{HendrycksD19,GeirhosRMBWB19,ZhuPIE17}. 
% As for text information, existing approaches usually perform character-, word-, or sentence-level perturbation on the text while assuring semantic equivalence  \cite{0002LSBLS18,LiuF021}.
% However, in multimodal tasks, information under different modalities is interrelated, and perturbation from information under only a single modality needs to consider the correctness of the perturbation, e.g., semantic equivalence perturbation in text.
% This leads to single-modal testing methods that could only perturb information at a shallow level, and thus detect limited issues with multimodal models.



As a fundamental task in the multimodal learning field, Visual Grounding (VG) aims to locate the object in an image through natural language expressions~\cite{mao2016generation,yang2022improving}, and it affects many downstream tasks such as Visual Question Answering (VQA)~\cite{antol2015vqa, das2018embodied}, 3D Visual Grounding ~\cite{liu2021refer, yuan2021instancerefer}, robot navigation ~\cite{qi2020reverie,anderson2018vision}, autonomous driving ~\cite{kim2019grounding} and photo editing~\cite{cheng2014imagespirit,Turmukhambetov16}.
Accordingly, the quality issues of the VG models have also attracted more and more attention.
For instance, Akula et al. \cite{AkulaGAZR20} reported that with subtle manual changes in the linguistic structure of the original expressions, the performance of the VG models will obviously decrease.
However, to our best knowledge, there are no automatic approaches specific to the VG models in the literature. 
How to automatically detect the quality issues for the VG models and improve their performance is a promising and unexplored research topic.


% Visual Grounding (VG) is a challenging and attractive task among multimodal tasks that requires model understanding and reasoning about semantics-rich natural language expressions and diverse image content \cite{karpathy2015deep,wang2016learning,yang2020graph}.
% Given an image and a text expression, VG aims to locate the object or region referred to in an image through natural language expression \cite{mao2016generation,yang2022improving}.
% VG is important for downstream tasks such as Visual Question Answering (VQA) \cite{antol2015vqa, das2018embodied} and 3D Visual Grounding \cite{liu2021refer, yuan2021instancerefer}, and its applications are widely explored in human daily life, such as robot navigation \cite{qi2020reverie,anderson2018vision}, autonomous driving \cite{kim2019grounding} and photo editing \cite{cheng2014imagespirit,Turmukhambetov16}.


%1. VG是一个什么样的任务（重点强调VG任务的输入），VG很重要；
% With the rapid development of multimodal learning techniques, many tasks have been able to be processed by the machine.
% Among them, Visual Grounding (VG) is a challenging and attractive task that requires machine understanding and reasoning about semantics-rich natural language expressions and diverse image content \cite{karpathy2015deep,wang2016learning,yang2020graph}.
% Given an image and a text expression, VG aims to locate the object or region referred to in an image through natural language expression \cite{mao2016generation,yang2022improving}.
% In recent years, VG has attracted a lot of attention since it has great potential to bridge the gap between linguistic expression and visual perception.
% The performance of VG has been improved tremendously with the rapid development of deep neural networks, for example, multimodal pre-training models \cite{lu2019vilbert, TanB19,su2019vl, LiDFGJ20,wang2022ofa} are able to extract and merge image and text features simultaneously and to accurately predict the regions corresponding to text in images by fine-tuning.
% VG is important for downstream tasks such as Visual Question Answering (VQA) \cite{antol2015vqa, das2018embodied} and 3D Visual Grounding \cite{liu2021refer, yuan2021instancerefer}, and its applications are widely explored in human daily life, such as robot navigation \cite{qi2020reverie,anderson2018vision}, autonomous driving \cite{kim2019grounding} and photo editing \cite{cheng2014imagespirit,Turmukhambetov16}.



%2. VG的质量问题，引出需要自动化方法去检测缺陷；
% However, despite its widespread adoption in various applications, the state-of-the-art VG model still mislocates the referred region of expression due to the complexity of the multimodal networks and text expression.
% Akula et al. \cite{AkulaGAZR20} found that the performance of the VG model on the new dataset decreases substantially after manually changing the linguistic structure of the original expressions.
% This indicates that the reliability of the VG model needs further validation, and therefore an automated test methodology is needed to detect issues with the VG model.

% 3. 作为VG一个重要的输入，expression的表述对VG models的性能有显著影响；

Metamorphic testing has been widely applied to test learning-based models to tackle the test oracle problem due to its simplicity of concept and effectiveness in fault detection~\cite{ChenKLPTTZ18}.
A central element of metamorphic testing is a set of Metamorphic Relations (MRs), which are necessary properties of the tested model in relation to the inputs and their expected outputs. 
Many approaches to testing the image-oriented or text-oriented deep learning models have designed the MRs by bringing a tiny perturbation for the inputs which keeps the original output oracle unchanged. 
% \rev{Generally, given the input and corresponding output oracle, existing testing methods for deep learning models follow the metamorphic relation}
% \jie{comment}
%这个说法感觉像是已有方法都是用的蜕变测试。其实是只有用蜕变测试的工作才会这样做，所以我修改了下。
% \rev{that generates the tests by perturbing the inputs without changing the original oracle.}
Given the two types of input (i.e., images and expressions) in the VG models, existing techniques can only carry out the perturbation either solely based on the image or solely on the natural language text. 
% \rev{for either image or natural language text may be borrowed for test generation.}
However, they could not be effectively used for VG models due to the following aspects.
\textbf{First}, for the images, traditional perturbation techniques usually introduce uncontrollable random noise with different granularities in images such as pixels and blocks or conduct unexplained image synthesis~\cite{HendrycksD19,GeirhosRMBWB19,ZhuPIE17}.
Based on the above implementation, some image features that have a significant impact on object location will undergo unpredictable changes before and after the perturbation, such as color and background (details are discussed in Section \ref{sec:analysis_img}), which leads to the changes of test oracles (i.e., the correct target region is changed).
% \jie{comment}
%能按照我上面说法吗？现在的the inability 不太清楚是要说明啥，是不是就是说这个修改改变了原来的ground truth了，所以其实是无效的。
% the inability of such perturbation techniques to be applied to test generation based on metamorphic relation.
\textbf{Second}, for natural language texts, most of the existing testing approaches (e.g., Q\&A system testing and translation system testing) conduct semantically-equivalent perturbations~\cite{SunZHPZ20,0004Z0HP022,RusertSS22}.
Specifically, given the original texts, they typically conduct synonym substitution, back translation, simulating some character-level spelling errors, or removing some uninformative words (e.g., adverbs and conjunctions) to ensure consistency in semantics before and after perturbation~\cite{0002LSBLS18,LiuF021}.
Generally, these semantically-equivalent perturbations are relatively subtle and shallow, which can hardly affect the issue detection ability of the automated testing approaches.
For the VG task, since both image and natural language text are entangled and interact with each other, we aim to conduct the perturbation by considering these two types of information.

% For VG models, it is valuable to design novel perturbation techniques for expressions via image understanding to improve the issue detection ability of the automated testing approaches.
% }

% The input to the VG model is multimodal information, and it is a challenge to combine image and text information for perturbation considering the limitations of existing methods for testing multimodal models.
% As a key input to the VG model, Expression has a significant impact on the performance of the VG model in terms of its formulation.
% 4. 引出一下有concise和precise的表达，说一下在VG任务下，consise和precise的定义是什么（比如有大于一个有判别性的features的expression叫做precise，只有唯一的判别性特征的expression是concise的）。举个例子说明VG model在处理concise和precise的expressions时候，性能有比较明显的差异（当然，如果有统计数据的支撑，更有说服力。如果没有的话，就用举例子的方式说吧）；
% \yuan{
% By the observation of the VG dataset, we found that the set of images in VG falls into two types: 1) Distinct Object Images, where the objects in the images are clearly distinguishable from each other. 2) Similar Object Images, where the objects in the images have a high degree of similarity to each other.
% Each image is typically described in two types of descriptive expressions, i.e., comprehensive expressions and concise expressions.
% In linguistics, comprehensive expressions tend to incorporate more abundant (and sometimes redundant) properties to describe an object ~\cite{hyland2007genre}.
% As for concise expressions, they aim to describe the object with fewer yet sufficient properties \cite{morkes1997concise,rowe2022concise}.
% For Distinct Object Images, where object features are easily recognizable, the VG model can precisely localize the object within the image through comprehensive or concise expressions.
% However, for Similar Object Images, there are multiple interference regions similar to the object region outside the object region in the image, and thus locating the object region requires more information for confirmation.
% Thus compared to the concise expression, the comprehensive expression is more helpful for the VG model to localize to the object region.
% As shown in Figure \ref{fig:motivation}, subfigure (a) shows the localization of the VG model under Distinct Object Images for the regions to concise and comprehensive expressions.
% Since the two kites in the image differ significantly in color features, the VG model is able to correctly locate the regions corresponding to the concise and comprehensive expressions.
% Subfigure (b) shows the localization of the VG model under Similar Object Images for the regions to concise and comprehensive expressions.
% Since the ``polar bear'' has regions of other objects with similar features to it in the image, a comprehensive expression containing more feature descriptions could help the VG model locate the correct region more accurately.
% Whereas a concise expression should theoretically be able to locate the correct region as well, the presence of interfering regions reduces the VG model's confidence in locating the correct region.
% This could potentially lead to incorrectly localizing an interfering region instead, as shown in subfigure (b).
% }

In linguistics, for an object, there are two types of descriptive expressions, i.e., comprehensive expressions and concise expressions~\cite{morkes1997concise,hyland2007genre,rowe2022concise}.
% Comprehensive expressions are likely to introduce more sufficient (sometimes redundant) features to describe the object while maintaining its accuracy, while concise expressions aim to describe the object with fewer features on the premise of accuracy.
Comprehensive expressions tend to incorporate more abundant (and sometimes redundant) properties to describe an object.
As for concise expressions, they aim to describe the object with fewer yet sufficient properties.
We demonstrate an example of these two types of expressions in the VG task.
Figure \ref{fig:motivation} shows a VG task aiming at locating the bird framed by the rectangle in the image.
By the image understanding, the framed bird can be located by either the position property ``standing behind two brown birds''  or the color property ``white''.
The comprehensive expression could be ``A white bird stands behind two brown birds'', while the concise expression could be ``A white bird'' or ``A bird stands behind two brown birds''.
\yuan{comment}
%根据王老师建议，我们将这一段还是改为信息熵的减少，但只说这是种引导模型出错的方法，不与compresive的进行对比
\yuan{
According to Shannon's Entropy theory~\cite{shannon2001mathematical}, the smaller amount of information an expression contains, the higher uncertainty is the expression. 
% This inspires us that a concise expression could induce the model to expose issues, and we design the perturbation techniques to transform comprehensive expressions into concise expressions to improve the issue detection ability for the VG models based on this assumption.
This inspires us that a concise expression could induce the VG model to expose issues. Therefore, under this assumption, we design perturbation techniques to convert comprehensive expressions into concise expressions, aiming to improve the issue detection ability for the VG models.
}
% , and will motivate our method design. 
% % \rev{The two types of expressions also exist in the VG task.}\jie{i feel like this sentence is useless, so i changed.}

% Although the two types of expression can both locate the object in the image for humans, they may have different effects on the VG models.
% \yuan{comment}
% %这里将之前的信息熵理论改为eccv一篇文章提到VG模型在编码整句时会忽略细节描述，由此在一些物体相似的图像下concise的表述会更容易出错，这里提出是在物体相似的图像下是因为在一些目标清晰的图像下例如只有一个物体（参见disccusion6.2中的示例）缩减句子并不会导致模型性能下降，因为本身图像就很容易区别，因此对这一问题做了情景的限制。
% \yuan{
% Specifically, according to Shannon's Entropy theory~\cite{shannon2001mathematical}, the smaller amount of information an expression contains, the higher uncertainty is the expression. 

% Specifically, according to the research conducted by Yang et al. \cite{YangC0L20}, the VG model is prone to overlook detailed descriptions in the expression when encoding the entire expression.
% However, when an object within an image significantly differs from the rest, this oversight does not impact the VG model's localization ability, as the core information\footnote{Words that describe the object itself, rather than its modifiers or detailed descriptions} conveyed in the expression is sufficient to help the model locate the object.
% On the other hand, in scenarios where an image contains multiple objects, and the target object shares similar characteristics with non-target objects, concise expressions are more likely to lead to model errors compared to comprehensive expressions, due to the inherent limitations of the VG model.
% % With comprehensive expressions, even after some features are ignored, the remaining features can still assist the VG model in accurately locating regions within the image. 
% % However, once key information from a concise expression is overlooked by the model, it becomes incapable of locating the original object.
% For example, in Figure \ref{fig:motivation}, there are multiple similarly shaped birds in the input image, and more description is needed to accurately locate one of them.
% As for comprehensive expression, the VG model can still locate the correct object guided by the remaining feature ``stands behind two brown birds'', even after overlooking the feature ``white'' from the whole expression.
% In contrast, when the feature ``white'' is overlooked during the encoding of the concise expression ``a white bird'', leaving only the meaning of ``bird'', the VG model fails to determine the exact location of the original object.
% % Specifically, according to Shannon's Entropy theory~\cite{shannon2001mathematical}, the smaller amount of information an expression contains, the higher uncertainty is the expression. 
% % For the VG task, compared with the comprehensive expressions, the VG models receive less information through the concise expressions and might have higher possibilities in exposing the issues.
% Therefore, it is potential to design the perturbation techniques to transform comprehensive expressions into concise expressions to improve the issue detection ability for the VG models.
% }

The biggest challenge to performing the expression transformation is how to find the concise expression that describes the original object and there are no other objects that satisfy the description, i.e., the test oracle (target region) remains unchanged.
To tackle this, we find the expression would involve the described ``object'' and several  ``properties'' as mentioned above, e.g., color, shape, wear, action, mood, location, etc.
By referring to the object together with some of its properties, we can potentially obtain several candidate concise expressions. 
We would then utilize the semantics of the image to determine whether a candidate concise expression can uniquely describe the target object, which can make better use of the two modes of information in the multimodal model.


% \rev{There are two challenges when performing the expression transformation for the VG task.}
% \jie{comment}
%我觉得这个challenges有点太细节了，感觉已经到怎么做的层面了。我也可能不用区分这个什么啊。我觉得这里应该还是先高层一点说吧，就是怎么着生成这些潜在的concise expression，以及需要保持oracle不变。
% \rev{\textbf{First}, to transform the precise into concise, it is vital to identify the ``object'' and corresponding ``properties'' from the original expression.  
% Especially, the object in an image usually has a wide variety of properties categories, e.g., color, shape, wear, action, mood, location, etc.
% Due to the various descriptive characteristics, the properties are far from being identified with some pre-defined linguistic patterns.
% How to identify the ``object'' and corresponding ``properties'' remains a challenge for the expression transformation.
% \textbf{Second}, given an object and property(s) in the precise expression, the transformation does not represent the arbitrary combination of them.
% In some cases, the arbitrary combinations may lead to changes in located targets, which cannot guarantee the oracle invariance in the metamorphic relation.
% How to determine whether the transformed concise expression can still locate the target image is the basis for ensuring automated testing approaches.}



% In text writing, there is often a tendency to express the text more precisely and concisely \cite{morkes1997concise,parnas2011precise,hotaling2020simple}.
% % Precise expression means that the meaning of the expression is complete and no ambiguous, while concise expression puts more emphasis on conveying ideas as clearly as possible with fewer words.
% While in VG task, the precise expression is to have as many modifiers as possible to describe  the target of the region referred to on the image, and the concise expression is to accurately refer to the region of the image with as fewer modifiers. 
% As shown in Figure \ref{fig:motivation}, in addition to the location information description (standing behind the two birds), the precise expression modifies the object (bird) with a color (white).
% In information theory Shannon's entropy theory reveals that the smaller the amount of information, the higher the uncertainty \cite{shannon2001mathematical}. 
% Inspired by the theory, we assume that the concise expression is more likely to make the model mislocalize regions than the precise expression in the VG task. 
% Therefore, we would like to transform the precise expression into the concise expression for detecting issues of the VG model.
% However, there are two challenges with such a text perturbation approach.
% The first challenge is that the modifiers in the expression need to be accurately identified, otherwise the semantics of the expression after deletion of the modifiers does not make sense. 
% The second challenge is that the expression after the deletion of the modifiers could still be located to the referred region on the image, which requires combining the image information.

%有很多方法以及数据集被提出，但缺乏VG的测试方法，现有的只有CV以及NLP的方法

In this paper, we propose an image-aware text perturbation approach (named {\tool}) for VG testing.
Under the framework of metamorphic testing, {\tool} introduces two metamorphic relations for expressions, i.e., image-aware concise expression transformation and semantically-equivalent expression transformation.
Specifically, through object/property extraction, recombination, and image-aware concise expression selection, {\tool} transforms the expressions into concise ones that can still locate the original target region on the image.
% \yang{TBD.}
% Its core idea is that the VG model should locate the original target region on the image if we could find an alternative (concise) expression that describes the original object and there is no other object satisfy the description. 
% To achieve this, {\tool} first trains a model to extract the object and corresponding properties in the expressions, and restructures them into candidate concise expressions. 
% For each candidate, {\tool} then designs three MR-related queries with image understanding, in order to validate whether the concise expression can uniquely describe the object in the original target region, i.e., test oracle keeps unchanged. 
% By querying the image with VQA model, the satisfied concise expression is found. 
Additionally, {\tool} further conducts semantically-equivalent perturbations, and generates the final perturbed expressions for VG testing.


% \rev{wo Metamorphic Relations (MRs) for testing visual grounding by image-aware text perturbation approach (named {\tool}).}
% \yang{Revise the following statements.}
% \rev{
% First, to achieve the image-aware concise expression transformation MR, {\tool} trains a model to identify the object to be located and corresponding properties in the expressions. 
% Then, the object and properties are restructured into candidate concise expressions.
% For each candidate concise expression, {\tool} has designed three MR-related query 
%  for asking whether the target region described in the concise expression is consistent with the original target region.
% Finally, {\tool} queries the image with the VQA model to confirm the satisfactory concise expression.
%  % , where the satisfactory concise expressions are discriminated by comparing the model's answers with the responses that are expected to indicate the uniqueness of the referred region.
% Second, to achieve the Semantically-equivalent expression transformation MR, {\tool} perturbs concise expressions with three widely-used semantically-equivalent textual perturbation methods, ultimately generating a test suite for testing VG models.
% }
% Then, the semantic components are restructured into concise expressions and {\tool} combines the concise expressions with manually designed question templates, which ask whether the referred region described in the concise expression is uniquely present in the image.


%0.1517-0.2776
We evaluate the issue detection capability of {\tool} on three publicly available VG datasets, i.e., RefCOCO \cite{YuPYBB16}, RefCOCO+ \cite{YuPYBB16} and RefCOCOg \cite{MaoHTCY016}.
%需要重新统计
Results show that, with the tests generated by {\tool}, the relative performance drop of OFA achieves 21.4\% in MultiModal Impact score (MMI), and outperforms state-of-the-art baselines for images and texts by 8.2\%--15.1\%.
In addition, perturbed expressions generated by the two MRs, i.e. Image-aware Concise Expression Transformation and Semantically-equivalent Expression Transformation, could respectively reach an MMI of 11.1\% and 14.2\% on average. 
Furthermore, the performance of the VG model can be enhanced by fine-tuning it using the tests generated by {\tool}.
The key contributions of this paper are as follows:
\begin{itemize}
    \item
    % \yuan{We propose a novel testing approach, {\tool}, to automatically detect the issues for VG models with the help of concise expression transformation and Semantically-equivalent expression perturbation.}
    We propose a text perturbation approach for visual grounding testing by designing the image-aware metamorphic relations with an image understanding technique. 
    This is the first approach for testing the VG model considering the two involved modes (image and text), to the best of our knowledge, and can motivate other research related to multimodal learning models. 
    
    % \item 
    % \yuan{
    % We design and implement two image-aware text metamorphic relations in {\tool}. 
    % {\tool} verifies the equivalence of test oracles by combining the semantics of the image and expression.
    % }
    % \jie{comment}
    %感觉第二个和第一个很类似，区分不出来。

    % is the testing approach correct? 
    % We propose a new testing approach, {\tool}, to automatically detect the issues in the VG model, in addition to the first attempt to combine image content with text perturbation for VG task.
    
    % \yang{
    % Different from the previous studies, we design an image-aware text perturbation for the expression in the VG task.
    % Combined with the general semantically-equivalent perturbation, {\tool} could improve the issue detection ability for the VG models.}
    
    % We propose a VG-oriented entity extraction model containing two categories of entities, which dissects the input text into multiple semantically integrated sentences for subsequent text deletion.
    \item 
    We perform comprehensive experiments to evaluate the effectiveness of {\tool}, the experimental results show that {\tool} can obviously improve the issue detection ability and significantly outperforms the state-of-the-art baselines on the MMI across three widely used datasets.
    
    \item
    By fine-tuning the original model with the generated tests, the performance of the VG model could be significantly improved.
   
    \item
    We provide the public reproduction package\footnote{https://github.com/IMGAT/IMGAT} including the tool implementation and datasets.
\end{itemize}




































==> tab/entity_and_improveacc.tex <==
\begin{table}[t]

\label{tab:entity_extraction}
\centering
\begin{minipage}{0.2\textwidth}
\begin{tabular}{c|ccccc}
\toprule
\textbf{Category}  & \textbf{Precision} & \textbf{Recall} & \textbf{F1} \\ \midrule
Object  & 94.9\%  & 93.8\%  & 94.3\%     \\
Property & 81.9\%  & 74.8\%  & 78.2\%    \\

                    
\bottomrule
\end{tabular}
\caption{Object and property extraction performance}
\end{minipage}

\hfill
\begin{minipage}{0.7\textwidth}
\label{tab:rq3}

\begin{tabular}{c|ccc}
\toprule
\textbf{Test Model} & \textbf{RefCOCO} & \textbf{RefCOCO+} & \textbf{RefCOCOg} \\ \midrule

Original model &   63.5\%     &   60.1\%     &   74.8\%     \\


Fine-tuned model  & 67.6\% ($\uparrow 6.4\%$)  & 68.9\% ($\uparrow 14.6\%$) &   76.0\% ($\uparrow 1.6\%$)   \\ 


\bottomrule
\end{tabular}
\caption{Improved accuracy after fine-tuning with tests generated by {\tool}}
\end{minipage}
\end{table}

==> tab/entity_extraction_discussion.tex <==
\begin{table}[t]
\small
\caption{VG-Oriented entity extraction performance under different sizes of training samples}
\label{tab:entity_extraction}
\centering
\resizebox{0.8\columnwidth}{!}{
\begin{tabular}{ccccc}
\toprule
K\%  & \textbf{25\%} & \textbf{50\%} & \textbf{75\%} &\textbf{100\%}  \\ \midrule
Precision & 82.5\%  & 85.9\%  & 87.9\%  & 88.4\%    \\
Recall  & 60.6\%  & 79.5\%  & 77.0\%  & 84.3\%      \\
F1  & 69.1\%  & 82.6\%  & 82.1\%  & 86.3\%    \\                      

\bottomrule
\end{tabular}
}
\end{table}
